PrivaScissors: Enhance the Privacy of Collaborative Inference through the Lens of Mutual Information

Edge-cloud collaborative inference empowers resource-limited IoT devices to support deep learning applications without disclosing their raw data to the cloud server, thus preserving privacy. Nevertheless, prior research has shown that collaborative inference still results in the exposure of data and predictions from edge devices. To enhance the privacy of collaborative inference, we introduce a defense strategy called PrivaScissors, which is designed to reduce the mutual information between a model's intermediate outcomes and the device's data and predictions. We evaluate PrivaScissors's performance on several datasets in the context of diverse attacks and offer a theoretical robustness guarantee.

==> method_bak.tex <==
\section{Method}

\subsection{Defense against IP leakage from mutual information perspective (DIMIP)}

Without loss of generality, we formulate our defense named DIMIP in the two-party scenario. Suppose the passive party (party 2) and active party (party 1) have sample pairs $\left\{\left(x_i^1, x_i^2, y_i\right)\right\}_{i=1}^N$ drawn from a distribution $p\left(x^1, x^2, y\right)$, and the representations of party $k$ is calculated as $h^k=f_{\theta_k}(x^k)$. We use $h^k$, $x^k$ and $y$ here to represent random variables, while $H_i^k$, $x_i^k$ and $y_i$ stand for deterministic values. Then our learning algorithm is to achieve two goals:

\begin{itemize}
    \item Goal 1: To preserve the performance of VFL, the main objective loss should be minimized.
    \item Goal 2: To reduce the IP leakage of labels from party 2, $\theta_2$ should not be able to extract representations $h^2$ containing much information about the true label $y$.
\end{itemize}


\noindent Formally, we have two training objectives:

\begin{equation}
    \begin{aligned}
    &\textbf{Prediction:} \min\limits_{\theta_1, \theta_2, \theta_S} \mathcal{L}\left(\mathcal{S}_{\theta_{\mathcal{S}}}\left(h^1, h^2\right), y\right),\\
    &\textbf{Label IP protection:} \min\limits_{\theta_2} \text{I}(h^2;y),
    \end{aligned}
\end{equation}

\noindent where $\text{I}(h^2;y)$ is the mutual information between $h^2$ and $y$, which indicates the information $h^2$ preserves for the label variable $y$. We minimize this mutual information to protect the active party's labels' IP from being learned by the passive party. Ideally, if the $\text{I}(h^2;y)=0$, no label can be inferred by the passive party.
%and the passive party has to pay effort to annotate a large amount of data after the termination of collaboration if it wants to provide service similar with the active party.

The prediction objective is usually easy to calculate (e.g., cross-entropy loss for classification). The mutual information term is hard to compute in practice as the random variable $h^2$ is high-dimensional. In addition, the mutual information requires knowing the distribution $p(y|h^2)$, which is difficult to compute. To derive a tractable estimation of the mutual information objective, we leverage \textit{CLUB}~\cite{cheng2020club} to formulate a variational upper-bound:

{\small
\begin{equation}
    \begin{aligned}
        &\text{I}\left(h^2;y\right)\\
        \leq~& \text{I}_\text{{vCLUB}}\left(h^2;y\right)\\
        :=~& \mathbb{E}_{p\left(h^2, y\right)}\log q_{\psi}\left(y|h^2\right)-\mathbb{E}_{p\left(h^2\right)p\left(y\right)}\log q_{\psi}\left(y|h^2\right),
    \end{aligned}
    \label{eq:vclub}
\end{equation}
}%

\noindent where $q_{\psi}\left(y|h^2\right)$ is a variational distribution with parameters $\psi$ to approximate $p\left(y|h^2\right)$. To reduce the computational overhead of the defense, we apply the sampled vCLUB (vCLUB-S) MI estimator in \cite{cheng2020club}, which is an unbiased estimator of $\text{I}_\text{{vCLUB}}$ and is formulated as
{\small
\begin{equation}
    \hat{\text{I}}_{\text{vCLUB-S}}(h^2;y) = \frac{1}{N} \sum\limits_{i=1}^N \left[\log q_{\psi}\left(y_i|H_i^2\right) - \log q_{\psi}\left(y_{k_i'}|H_i^2\right)\right],
\label{eq:vclubs}
\end{equation}
}%

\noindent where $k_i'$ is uniformly sampled from indices $\{1,...,N\}$. It is notable that to guarantee the first inequality of \cref{eq:vclub}, $q_{\psi}\left(y|h^2\right)$ should satisfy 

{\small
\begin{equation}
    \text{KL}\left(p\left(h^2,y\right)||q_\psi\left(h^2,y\right)\right)\leq \text{KL}\left(p\left(h^2\right)p\left(y\right)||q_\psi\left(h^2,y\right)\right),
\end{equation}
}
\noindent which can be achieved by minimizing $\text{KL}\left(p\left(h^2,y\right)||q_\psi\left(h^2,y\right)\right)$:

{\small
\begin{equation}
    \begin{aligned}
        &\min\limits_\psi \text{KL}\left(p\left(h^2,y\right)||q_\psi\left(h^2,y\right)\right)\\
        =~&\min\limits_\psi \mathbb{E}_ {p\left(h^2,y\right)}\left[\log\left(p\left(y|h^2\right)p\left(h^2\right)\right)-\log\left(q_{\psi}\left(y|h^2\right)p\left(h^2\right)\right)\right]\\
        =~&\min\limits_\psi \mathbb{E}_ {p\left(h^2,y\right)}\left[\log\left(p\left(y|h^2\right)\right)-\log\left(q_{\psi}\left(y|h^2\right)\right)\right].
    \end{aligned}
\end{equation}
}%

\noindent Since the first term has no relation to $\psi$, we just need to minimize $\mathbb{E}_ {p\left(h^2,y\right)}-\log\left(q_{\psi}\left(y|h^2\right)\right)$. With samples $\left\{\left(x_i^1, x_i^2, y_i\right)\right\}_{i=0}^N$, we can derive an unbiased estimation 

{\small
\begin{equation}
    \max\limits_{\psi}\frac{1}{N} \sum\limits_{i=1}^N \log q_{\psi}\left(y_i|H_i^2\right).
\label{eq:condition}
\end{equation}
}%

\noindent With \cref{eq:vclub}, \cref{eq:vclubs} and \cref{eq:condition}, the objective of label IP protection can be achieved by optimizing

{\small
\begin{equation}
    \begin{aligned}
        &\min\limits_{\theta_2} \text{I}(h^2;y)\\
        \Leftrightarrow~&\min\limits_{\theta_2} \hat{\text{I}}_{\text{vCLUB-S}}(h^2;y)\\
        =~&\min\limits_{\theta_2} \frac{1}{N} \sum\limits_{i=1}^N \left[\max\limits_{\psi}\log q_{\psi}\left(y_i|H_i^2\right) - \log q_{\psi}\left(y_{k_i'}|H_i^2\right)\right].
    \end{aligned}
    \label{eq:variational_objective}
\end{equation}
}%

\noindent Suppose we use $g_{\psi}$ to parameterize $q_{\psi}$, by combining \cref{eq:variational_objective} and the prediction objective with a weight hyper-parameter $\lambda$, we formulate the overall optimizing objective as

% {\small
% \begin{equation}
%     \begin{aligned}
%         &\min\limits_{\theta_1, \theta_2, \theta_S}(1-\lambda)\underbrace{\frac{1}{N} \sum_{i=1}^{N} \text{CE}\left(\mathcal{S}_{\theta_{\mathcal{S}}}\left(f_{\theta_1}\left(x_i^1\right),f_{\theta_2}\left(x_i^2\right)\right), y_i\right)}_{L_C}\\
%         &+\min\limits_{\theta_2}\max\limits_{\psi} \lambda\underbrace{\frac{1}{N} \sum\limits_{i=1}^N -\text{CE} \left(g_{\psi}\left(f_{\theta_2}\left(x_i^2\right)\right),y_i\right)}_{L_A}\\
%         &+\min\limits_{\theta_2} \lambda\underbrace{\frac{1}{N} \sum\limits_{i=1}^N\text{CE} \left(g_{\psi}\left(f_{\theta_2}\left(x_i^2\right)\right),y_{k_i'}\right)}_{L_R}.
%         \label{eq:final_object}
%     \end{aligned}
% \end{equation}
% }%

{\small
\begin{equation}
    \begin{aligned}
        &\min\limits_{\theta_1, \theta_2, \theta_S}(1-\lambda)\underbrace{\frac{1}{N} \sum_{i=1}^{N} \mathcal{L} \left(\mathcal{S}_{\theta_{\mathcal{S}}}\left(f_{\theta_1}\left(x_i^1\right),f_{\theta_2}\left(x_i^2\right)\right), y_i\right)}_{\mathcal{L}_C}\\
        &+\min\limits_{\theta_2}\max\limits_{\psi} \lambda\underbrace{\frac{1}{N} \sum\limits_{i=1}^N \log g_{\psi}\left(y_i|f_{\theta_2}\left(x_i^2\right)\right)}_{\mathcal{L}_A}\\
        &+\min\limits_{\theta_2} \lambda\underbrace{\frac{1}{N} \sum\limits_{i=1}^N-\log g_{\psi}\left(y_{k_i'}|f_{\theta_2}\left(x_i^2\right)\right)}_{\mathcal{L}_R}.
        \label{eq:final_object}
    \end{aligned}
\end{equation}
}%
